L2 Regularization versus Batch and Weight Normalization

Batch Normalization is a commonly used trick to improve the training of deep neural networks. These neural networks use L2 regularization, also called weight decay, ostensibly to prevent overfitting. However, we show that L2 regularization has no regularizing effect when combined with normalization. Instead, regularization has an influence on the scale of weights, and thereby on the effective learning rate. We investigate this dependence, both in theory, and experimentally. We show that popular optimization methods such as ADAM only partially eliminate the influence of normalization on the learning rate. This leads to a discussion on other ways to mitigate this issue.

==> best_learning_rate_adam_weights_only.tex <==
0.000001 0.020000
0.000010 0.005000
0.000100 0.002000
0.001000 0.001000
0.010000 0.000500
0.100000 0.000200
1.000000 0.000100


==> best_learning_rate_nesterov_weights_only.tex <==
0.000001 0.050000
0.000010 0.200000
0.000100 0.200000
0.001000 0.020000
0.010000 0.002000
0.100000 0.000200
1.000000 0.000100


==> best_learning_rate_rmsprop_weights_only.tex <==
0.000001 0.005000
0.000010 0.010000
0.000100 0.002000
0.001000 0.001000
0.010000 0.000500
0.100000 0.000200
1.000000 0.000100


==> best_learning_rate_sgd_weights_only.tex <==
0.000001 0.500000
0.000010 2.000000
0.000100 2.000000
0.001000 0.100000
0.010000 0.050000
0.100000 0.002000
1.000000 0.000500


==> best_test_error_normalize_nesterov_weights_only.tex <==
0.000001 13.110978
0.000010 14.553285
0.000100 13.331330
0.001000 13.311298
0.010000 13.581731
0.100000 13.561699
1.000000 14.943910


==> best_test_error_normalize_rmsprop_weights_only.tex <==
0.000001 13.591747
0.000010 13.201122
0.000100 13.151042
0.001000 13.681891
0.010000 15.014022
0.100000 18.729968
1.000000 27.714343


==> test_error_adam_weights_only.tex <==
3.16228e-07 7.07107e-05 0.187901
3.16228e-07 0.000141421 0.164964
3.16228e-07 0.000353553 0.148738
3.16228e-07 0.000707107 0.145333
3.16228e-07 0.00141421 0.146835
3.16228e-07 0.00353553 0.142829
3.16228e-07 0.00707107 0.140525
3.16228e-07 0.0141421 0.141526
3.16228e-07 0.0353553 0.150541
3.16228e-07 0.0707107 0.159856
3.16228e-07 0.141421 0.166567
3.16228e-07 0.353553 0.170773
3.16228e-07 0.707107 0.176583
3.16228e-07 1.41421 0.175681
3.16228e-07 3.53553 0.185497
3.16228e-07 7.07107 0.185497

3.16228e-06 7.07107e-05 0.189002
3.16228e-06 0.000141421 0.165966
3.16228e-06 0.000353553 0.147035
3.16228e-06 0.000707107 0.144832
3.16228e-06 0.00141421 0.138421
3.16228e-06 0.00353553 0.139223
3.16228e-06 0.00707107 0.134215
3.16228e-06 0.0141421 0.141026
3.16228e-06 0.0353553 0.163862
3.16228e-06 0.0707107 0.210938
3.16228e-06 0.141421 0.263021
3.16228e-06 0.353553 0.43129
3.16228e-06 0.707107 0.816106
3.16228e-06 1.41421 0.441106
3.16228e-06 3.53553 0.915565
3.16228e-06 7.07107 0.915565

3.16228e-05 7.07107e-05 0.189403
3.16228e-05 0.000141421 0.159555
3.16228e-05 0.000353553 0.154046
3.16228e-05 0.000707107 0.138421
3.16228e-05 0.00141421 0.134215
3.16228e-05 0.00353553 0.140124
3.16228e-05 0.00707107 0.154848
3.16228e-05 0.0141421 0.172476
3.16228e-05 0.0353553 0.245593
3.16228e-05 0.0707107 0.332432
3.16228e-05 0.141421 0.394631
3.16228e-05 0.353553 0.519331
3.16228e-05 0.707107 0.89994
3.16228e-05 1.41421 0.89994
3.16228e-05 3.53553 0.885016
3.16228e-05 7.07107 0.885016

0.000316228 7.07107e-05 0.180789
0.000316228 0.000141421 0.157552
0.000316228 0.000353553 0.139223
0.000316228 0.000707107 0.13772
0.000316228 0.00141421 0.136118
0.000316228 0.00353553 0.163261
0.000316228 0.00707107 0.205629
0.000316228 0.0141421 0.256711
0.000316228 0.0353553 0.384215
0.000316228 0.0707107 0.398538
0.000316228 0.141421 0.540565
0.000316228 0.353553 0.899639
0.000316228 0.707107 0.72506
0.000316228 1.41421 0.852664
0.000316228 3.53553 0.898538
0.000316228 7.07107 0.898538

0.00316228 7.07107e-05 0.158654
0.00316228 0.000141421 0.138121
0.00316228 0.000353553 0.136719
0.00316228 0.000707107 0.14363
0.00316228 0.00141421 0.179888
0.00316228 0.00353553 0.261619
0.00316228 0.00707107 0.316506
0.00316228 0.0141421 0.460537
0.00316228 0.0353553 0.545373
0.00316228 0.0707107 0.714643
0.00316228 0.141421 0.89984
0.00316228 0.353553 0.897536
0.00316228 0.707107 0.836238
0.00316228 1.41421 0.892528
0.00316228 3.53553 0.891026
0.00316228 7.07107 0.891026

0.0316228 7.07107e-05 0.135016
0.0316228 0.000141421 0.136819
0.0316228 0.000353553 0.163762
0.0316228 0.000707107 0.211438
0.0316228 0.00141421 0.278846
0.0316228 0.00353553 0.373097
0.0316228 0.00707107 0.547276
0.0316228 0.0141421 0.57482
0.0316228 0.0353553 0.797175
0.0316228 0.0707107 0.80649
0.0316228 0.141421 0.806791
0.0316228 0.353553 0.90014
0.0316228 0.707107 0.8122
0.0316228 1.41421 0.90014
0.0316228 3.53553 0.89984
0.0316228 7.07107 0.89984

0.316228 7.07107e-05 0.136218
0.316228 0.000141421 0.163361
0.316228 0.000353553 0.241486
0.316228 0.000707107 0.313902
0.316228 0.00141421 0.390725
0.316228 0.00353553 0.462139
0.316228 0.00707107 0.851963
0.316228 0.0141421 0.821114
0.316228 0.0353553 0.78736
0.316228 0.0707107 0.889123
0.316228 0.141421 0.899139
0.316228 0.353553 0.854367
0.316228 0.707107 0.89994
0.316228 1.41421 0.90014
0.316228 3.53553 0.89984
0.316228 7.07107 0.89984

3.16228 7.07107e-05 0.136218
3.16228 0.000141421 0.163361
3.16228 0.000353553 0.241486
3.16228 0.000707107 0.313902
3.16228 0.00141421 0.390725
3.16228 0.00353553 0.462139
3.16228 0.00707107 0.851963
3.16228 0.0141421 0.821114
3.16228 0.0353553 0.78736
3.16228 0.0707107 0.889123
3.16228 0.141421 0.899139
3.16228 0.353553 0.854367
3.16228 0.707107 0.89994
3.16228 1.41421 0.90014
3.16228 3.53553 0.89984
3.16228 7.07107 0.89984



==> test_error_nesterov_weights_only.tex <==
3.16228e-07 7.07107e-05 0.311599
3.16228e-07 0.000141421 0.254407
3.16228e-07 0.000353553 0.207532
3.16228e-07 0.000707107 0.179087
3.16228e-07 0.00141421 0.165765
3.16228e-07 0.00353553 0.149639
3.16228e-07 0.00707107 0.149639
3.16228e-07 0.0141421 0.15004
3.16228e-07 0.0353553 0.149439
3.16228e-07 0.0707107 0.147135
3.16228e-07 0.141421 0.144932
3.16228e-07 0.353553 0.152644
3.16228e-07 0.707107 0.16226
3.16228e-07 1.41421 0.181591
3.16228e-07 3.53553 0.190605
3.16228e-07 7.07107 0.190605

3.16228e-06 7.07107e-05 0.314403
3.16228e-06 0.000141421 0.263121
3.16228e-06 0.000353553 0.205228
3.16228e-06 0.000707107 0.183193
3.16228e-06 0.00141421 0.156751
3.16228e-06 0.00353553 0.145733
3.16228e-06 0.00707107 0.142528
3.16228e-06 0.0141421 0.146735
3.16228e-06 0.0353553 0.143429
3.16228e-06 0.0707107 0.147135
3.16228e-06 0.141421 0.141126
3.16228e-06 0.353553 0.145933
3.16228e-06 0.707107 0.146234
3.16228e-06 1.41421 0.145032
3.16228e-06 3.53553 0.181791
3.16228e-06 7.07107 0.181791

3.16228e-05 7.07107e-05 0.313702
3.16228e-05 0.000141421 0.252304
3.16228e-05 0.000353553 0.211839
3.16228e-05 0.000707107 0.17478
3.16228e-05 0.00141421 0.164764
3.16228e-05 0.00353553 0.14383
3.16228e-05 0.00707107 0.14383
3.16228e-05 0.0141421 0.144331
3.16228e-05 0.0353553 0.139824
3.16228e-05 0.0707107 0.13772
3.16228e-05 0.141421 0.135417
3.16228e-05 0.353553 0.142528
3.16228e-05 0.707107 0.153646
3.16228e-05 1.41421 0.213742
3.16228e-05 3.53553 0.34385
3.16228e-05 7.07107 0.34385

0.000316228 7.07107e-05 0.310397
0.000316228 0.000141421 0.258113
0.000316228 0.000353553 0.197516
0.000316228 0.000707107 0.164864
0.000316228 0.00141421 0.151142
0.000316228 0.00353553 0.133514
0.000316228 0.00707107 0.133413
0.000316228 0.0141421 0.13772
0.000316228 0.0353553 0.142528
0.000316228 0.0707107 0.154547
0.000316228 0.141421 0.214744
0.000316228 0.353553 0.239583
0.000316228 0.707107 0.249299
0.000316228 1.41421 0.411158
0.000316228 3.53553 0.472456
0.000316228 7.07107 0.472456

0.00316228 7.07107e-05 0.283253
0.00316228 0.000141421 0.213141
0.00316228 0.000353553 0.148337
0.00316228 0.000707107 0.142228
0.00316228 0.00141421 0.136018
0.00316228 0.00353553 0.139123
0.00316228 0.00707107 0.147336
0.00316228 0.0141421 0.167067
0.00316228 0.0353553 0.23738
0.00316228 0.0707107 0.292167
0.00316228 0.141421 0.335938
0.00316228 0.353553 0.355068
0.00316228 0.707107 0.410056
0.00316228 1.41421 0.754607
0.00316228 3.53553 0.743389
0.00316228 7.07107 0.743389

0.0316228 7.07107e-05 0.145833
0.0316228 0.000141421 0.139123
0.0316228 0.000353553 0.144231
0.0316228 0.000707107 0.151542
0.0316228 0.00141421 0.170072
0.0316228 0.00353553 0.22486
0.0316228 0.00707107 0.35597
0.0316228 0.0141421 0.364683
0.0316228 0.0353553 0.481871
0.0316228 0.0707107 0.443009
0.0316228 0.141421 0.569211
0.0316228 0.353553 0.757111
0.0316228 0.707107 0.777845
0.0316228 1.41421 0.867388
0.0316228 3.53553 0.90014
0.0316228 7.07107 0.90014

0.316228 7.07107e-05 0.168269
0.316228 0.000141421 0.20613
0.316228 0.000353553 0.178986
0.316228 0.000707107 0.278646
0.316228 0.00141421 0.223458
0.316228 0.00353553 0.440104
0.316228 0.00707107 0.386118
0.316228 0.0141421 0.577724
0.316228 0.0353553 0.732171
0.316228 0.0707107 0.634014
0.316228 0.141421 0.750701
0.316228 0.353553 0.89984
0.316228 0.707107 0.90004
0.316228 1.41421 0.90004
0.316228 3.53553 0.90004
0.316228 7.07107 0.90004

3.16228 7.07107e-05 0.168269
3.16228 0.000141421 0.20613
3.16228 0.000353553 0.178986
3.16228 0.000707107 0.278646
3.16228 0.00141421 0.223458
3.16228 0.00353553 0.440104
3.16228 0.00707107 0.386118
3.16228 0.0141421 0.577724
3.16228 0.0353553 0.732171
3.16228 0.0707107 0.634014
3.16228 0.141421 0.750701
3.16228 0.353553 0.89984
3.16228 0.707107 0.90004
3.16228 1.41421 0.90004
3.16228 3.53553 0.90004
3.16228 7.07107 0.90004



==> test_error_normalize_nesterov_weights_only.tex <==
3.16228e-07 7.07107e-05 0.321514
3.16228e-07 0.000141421 0.248197
3.16228e-07 0.000353553 0.201422
3.16228e-07 0.000707107 0.170773
3.16228e-07 0.00141421 0.157151
3.16228e-07 0.00353553 0.141727
3.16228e-07 0.00707107 0.139123
3.16228e-07 0.0141421 0.13111
3.16228e-07 0.0353553 0.145833
3.16228e-07 0.0707107 0.149239
3.16228e-07 0.141421 0.213642
3.16228e-07 0.353553 0.184796
3.16228e-07 0.707107 0.306691
3.16228e-07 1.41421 0.38762
3.16228e-07 3.53553 0.748698
3.16228e-07 7.07107 0.748698

3.16228e-06 7.07107e-05 0.311599
3.16228e-06 0.000141421 0.260417
3.16228e-06 0.000353553 0.202524
3.16228e-06 0.000707107 0.173778
3.16228e-06 0.00141421 0.153646
3.16228e-06 0.00353553 0.145933
3.16228e-06 0.00707107 0.132111
3.16228e-06 0.0141421 0.145533
3.16228e-06 0.0353553 0.139623
3.16228e-06 0.0707107 0.147035
3.16228e-06 0.141421 0.165064
3.16228e-06 0.353553 0.196715
3.16228e-06 0.707107 0.311999
3.16228e-06 1.41421 0.35597
3.16228e-06 3.53553 0.60026
3.16228e-06 7.07107 0.60026

3.16228e-05 7.07107e-05 0.318009
3.16228e-05 0.000141421 0.254207
3.16228e-05 0.000353553 0.202224
3.16228e-05 0.000707107 0.169271
3.16228e-05 0.00141421 0.151242
3.16228e-05 0.00353553 0.142728
3.16228e-05 0.00707107 0.133313
3.16228e-05 0.0141421 0.134515
3.16228e-05 0.0353553 0.139724
3.16228e-05 0.0707107 0.145132
3.16228e-05 0.141421 0.165164
3.16228e-05 0.353553 0.202123
3.16228e-05 0.707107 0.292067
3.16228e-05 1.41421 0.465445
3.16228e-05 3.53553 0.553085
3.16228e-05 7.07107 0.553085

0.000316228 7.07107e-05 0.3126
0.000316228 0.000141421 0.263622
0.000316228 0.000353553 0.200721
0.000316228 0.000707107 0.173678
0.000316228 0.00141421 0.153646
0.000316228 0.00353553 0.14373
0.000316228 0.00707107 0.133113
0.000316228 0.0141421 0.134716
0.000316228 0.0353553 0.140224
0.000316228 0.0707107 0.151242
0.000316228 0.141421 0.183293
0.000316228 0.353553 0.280549
0.000316228 0.707107 0.255208
0.000316228 1.41421 0.445513
0.000316228 3.53553 0.564503
0.000316228 7.07107 0.564503

0.00316228 7.07107e-05 0.320413
0.00316228 0.000141421 0.264323
0.00316228 0.000353553 0.203826
0.00316228 0.000707107 0.171274
0.00316228 0.00141421 0.153746
0.00316228 0.00353553 0.141426
0.00316228 0.00707107 0.13762
0.00316228 0.0141421 0.135817
0.00316228 0.0353553 0.140725
0.00316228 0.0707107 0.173678
0.00316228 0.141421 0.177885
0.00316228 0.353553 0.244191
0.00316228 0.707107 0.261318
0.00316228 1.41421 0.414363
0.00316228 3.53553 0.791366
0.00316228 7.07107 0.791366

0.0316228 7.07107e-05 0.315705
0.0316228 0.000141421 0.255208
0.0316228 0.000353553 0.204627
0.0316228 0.000707107 0.171675
0.0316228 0.00141421 0.154948
0.0316228 0.00353553 0.135717
0.0316228 0.00707107 0.135617
0.0316228 0.0141421 0.140124
0.0316228 0.0353553 0.179688
0.0316228 0.0707107 0.215044
0.0316228 0.141421 0.282652
0.0316228 0.353553 0.597656
0.0316228 0.707107 0.520833
0.0316228 1.41421 0.608774
0.0316228 3.53553 0.886418
0.0316228 7.07107 0.886418

0.316228 7.07107e-05 0.307292
0.316228 0.000141421 0.249499
0.316228 0.000353553 0.194712
0.316228 0.000707107 0.170573
0.316228 0.00141421 0.149439
0.316228 0.00353553 0.16847
0.316228 0.00707107 0.222756
0.316228 0.0141421 0.181791
0.316228 0.0353553 0.188702
0.316228 0.0707107 0.333433
0.316228 0.141421 0.264724
0.316228 0.353553 0.676082
0.316228 0.707107 0.90014
0.316228 1.41421 0.857272
0.316228 3.53553 0.89994
0.316228 7.07107 0.89994

3.16228 7.07107e-05 0.307292
3.16228 0.000141421 0.249499
3.16228 0.000353553 0.194712
3.16228 0.000707107 0.170573
3.16228 0.00141421 0.149439
3.16228 0.00353553 0.16847
3.16228 0.00707107 0.222756
3.16228 0.0141421 0.181791
3.16228 0.0353553 0.188702
3.16228 0.0707107 0.333433
3.16228 0.141421 0.264724
3.16228 0.353553 0.676082
3.16228 0.707107 0.90014
3.16228 1.41421 0.857272
3.16228 3.53553 0.89994
3.16228 7.07107 0.89994



==> test_error_normalize_rmsprop_weights_only.tex <==
3.16228e-07 7.07107e-05 0.1874
3.16228e-07 0.000141421 0.161158
3.16228e-07 0.000353553 0.139022
3.16228e-07 0.000707107 0.135917
3.16228e-07 0.00141421 0.141226
3.16228e-07 0.00353553 0.149139
3.16228e-07 0.00707107 0.160457
3.16228e-07 0.0141421 0.208534
3.16228e-07 0.0353553 0.296675
3.16228e-07 0.0707107 0.472155
3.16228e-07 0.141421 0.514724
3.16228e-07 0.353553 0.75651
3.16228e-07 0.707107 0.90014
3.16228e-07 1.41421 0.89984
3.16228e-07 3.53553 0.90014
3.16228e-07 7.07107 0.90014

3.16228e-06 7.07107e-05 0.185897
3.16228e-06 0.000141421 0.158253
3.16228e-06 0.000353553 0.144431
3.16228e-06 0.000707107 0.132011
3.16228e-06 0.00141421 0.137921
3.16228e-06 0.00353553 0.145132
3.16228e-06 0.00707107 0.155248
3.16228e-06 0.0141421 0.191306
3.16228e-06 0.0353553 0.280449
3.16228e-06 0.0707107 0.405248
3.16228e-06 0.141421 0.697316
3.16228e-06 0.353553 0.797476
3.16228e-06 0.707107 0.90014
3.16228e-06 1.41421 0.89994
3.16228e-06 3.53553 0.90014
3.16228e-06 7.07107 0.90014

3.16228e-05 7.07107e-05 0.190204
3.16228e-05 0.000141421 0.162861
3.16228e-05 0.000353553 0.140725
3.16228e-05 0.000707107 0.13151
3.16228e-05 0.00141421 0.138522
3.16228e-05 0.00353553 0.147035
3.16228e-05 0.00707107 0.151242
3.16228e-05 0.0141421 0.197115
3.16228e-05 0.0353553 0.252404
3.16228e-05 0.0707107 0.402043
3.16228e-05 0.141421 0.618089
3.16228e-05 0.353553 0.637119
3.16228e-05 0.707107 0.89994
3.16228e-05 1.41421 0.89984
3.16228e-05 3.53553 0.89984
3.16228e-05 7.07107 0.89984

0.000316228 7.07107e-05 0.184495
0.000316228 0.000141421 0.163562
0.000316228 0.000353553 0.144131
0.000316228 0.000707107 0.136819
0.000316228 0.00141421 0.140124
0.000316228 0.00353553 0.148237
0.000316228 0.00707107 0.154046
0.000316228 0.0141421 0.197917
0.000316228 0.0353553 0.271835
0.000316228 0.0707107 0.501302
0.000316228 0.141421 0.680489
0.000316228 0.353553 0.680789
0.000316228 0.707107 0.90004
0.000316228 1.41421 0.89994
0.000316228 3.53553 0.90014
0.000316228 7.07107 0.90014

0.00316228 7.07107e-05 0.185797
0.00316228 0.000141421 0.160457
0.00316228 0.000353553 0.15014
0.00316228 0.000707107 0.16256
0.00316228 0.00141421 0.1876
0.00316228 0.00353553 0.242188
0.00316228 0.00707107 0.295873
0.00316228 0.0141421 0.355469
0.00316228 0.0353553 0.611278
0.00316228 0.0707107 0.611779
0.00316228 0.141421 0.61849
0.00316228 0.353553 0.877905
0.00316228 0.707107 0.90014
0.00316228 1.41421 0.89984
0.00316228 3.53553 0.89984
0.00316228 7.07107 0.89984

0.0316228 7.07107e-05 0.236078
0.0316228 0.000141421 0.1873
0.0316228 0.000353553 0.199219
0.0316228 0.000707107 0.249599
0.0316228 0.00141421 0.276943
0.0316228 0.00353553 0.427985
0.0316228 0.00707107 0.554688
0.0316228 0.0141421 0.70613
0.0316228 0.0353553 0.724359
0.0316228 0.0707107 0.892228
0.0316228 0.141421 0.741486
0.0316228 0.353553 0.782652
0.0316228 0.707107 0.90014
0.0316228 1.41421 0.90014
0.0316228 3.53553 0.91246
0.0316228 7.07107 0.91246

0.316228 7.07107e-05 0.360677
0.316228 0.000141421 0.277143
0.316228 0.000353553 0.294271
0.316228 0.000707107 0.360076
0.316228 0.00141421 0.417268
0.316228 0.00353553 0.515425
0.316228 0.00707107 0.634415
0.316228 0.0141421 0.744792
0.316228 0.0353553 0.701623
0.316228 0.0707107 0.729667
0.316228 0.141421 0.89984
0.316228 0.353553 0.90014
0.316228 0.707107 0.90014
0.316228 1.41421 0.90004
0.316228 3.53553 0.90014
0.316228 7.07107 0.90014

3.16228 7.07107e-05 0.360677
3.16228 0.000141421 0.277143
3.16228 0.000353553 0.294271
3.16228 0.000707107 0.360076
3.16228 0.00141421 0.417268
3.16228 0.00353553 0.515425
3.16228 0.00707107 0.634415
3.16228 0.0141421 0.744792
3.16228 0.0353553 0.701623
3.16228 0.0707107 0.729667
3.16228 0.141421 0.89984
3.16228 0.353553 0.90014
3.16228 0.707107 0.90014
3.16228 1.41421 0.90004
3.16228 3.53553 0.90014
3.16228 7.07107 0.90014



==> weight_norm_adam_weights_only.tex <==
3.16228e-07 7.07107e-05 0.387045
3.16228e-07 0.000141421 0.431789
3.16228e-07 0.000353553 0.601749
3.16228e-07 0.000707107 0.827493
3.16228e-07 0.00141421 1.10852
3.16228e-07 0.00353553 1.49761
3.16228e-07 0.00707107 1.79017
3.16228e-07 0.0141421 2.07475
3.16228e-07 0.0353553 2.42043
3.16228e-07 0.0707107 2.60643
3.16228e-07 0.141421 2.87423
3.16228e-07 0.353553 3.2363
3.16228e-07 0.707107 3.52471
3.16228e-07 1.41421 3.8792
3.16228e-07 3.53553 4.2331
3.16228e-07 7.07107 4.2331

3.16228e-06 7.07107e-05 0.379752
3.16228e-06 0.000141421 0.429984
3.16228e-06 0.000353553 0.597529
3.16228e-06 0.000707107 0.822186
3.16228e-06 0.00141421 1.07952
3.16228e-06 0.00353553 1.33559
3.16228e-06 0.00707107 1.45841
3.16228e-06 0.0141421 1.53828
3.16228e-06 0.0353553 1.62142
3.16228e-06 0.0707107 1.61373
3.16228e-06 0.141421 1.66274
3.16228e-06 0.353553 1.71736
3.16228e-06 0.707107 1.68241
3.16228e-06 1.41421 1.74978
3.16228e-06 3.53553 1.87303
3.16228e-06 7.07107 1.87303

3.16228e-05 7.07107e-05 0.381571
3.16228e-05 0.000141421 0.419171
3.16228e-05 0.000353553 0.580025
3.16228e-05 0.000707107 0.772128
3.16228e-05 0.00141421 0.940191
3.16228e-05 0.00353553 1.04396
3.16228e-05 0.00707107 1.08625
3.16228e-05 0.0141421 1.09056
3.16228e-05 0.0353553 1.14537
3.16228e-05 0.0707107 1.17341
3.16228e-05 0.141421 1.23259
3.16228e-05 0.353553 1.23986
3.16228e-05 0.707107 1.29225
3.16228e-05 1.41421 1.33265
3.16228e-05 3.53553 1.76435
3.16228e-05 7.07107 1.76435

0.000316228 7.07107e-05 0.356576
0.000316228 0.000141421 0.38027
0.000316228 0.000353553 0.460621
0.000316228 0.000707107 0.531211
0.000316228 0.00141421 0.57227
0.000316228 0.00353553 0.602066
0.000316228 0.00707107 0.631486
0.000316228 0.0141421 0.657982
0.000316228 0.0353553 0.665138
0.000316228 0.0707107 0.756705
0.000316228 0.141421 0.699161
0.000316228 0.353553 0.552822
0.000316228 0.707107 0.881775
0.000316228 1.41421 1.14638
0.000316228 3.53553 1.24022
0.000316228 7.07107 1.24022

0.00316228 7.07107e-05 0.214027
0.00316228 0.000141421 0.126623
0.00316228 0.000353553 0.099594
0.00316228 0.000707107 0.115962
0.00316228 0.00141421 0.142017
0.00316228 0.00353553 0.161007
0.00316228 0.00707107 0.192911
0.00316228 0.0141421 0.204172
0.00316228 0.0353553 0.263411
0.00316228 0.0707107 0.194597
0.00316228 0.141421 0.0842904
0.00316228 0.353553 0.876345
0.00316228 0.707107 0.886706
0.00316228 1.41421 0.777624
0.00316228 3.53553 1.37459
0.00316228 7.07107 1.37459

0.0316228 7.07107e-05 -0.34797
0.0316228 0.000141421 -0.363042
0.0316228 0.000353553 -0.352241
0.0316228 0.000707107 -0.333146
0.0316228 0.00141421 -0.310361
0.0316228 0.00353553 -0.302566
0.0316228 0.00707107 -0.278225
0.0316228 0.0141421 -0.323039
0.0316228 0.0353553 -0.287805
0.0316228 0.0707107 0.455808
0.0316228 0.141421 0.0453373
0.0316228 0.353553 0.170648
0.0316228 0.707107 0.494784
0.0316228 1.41421 0.551424
0.0316228 3.53553 1.26951
0.0316228 7.07107 1.26951

0.316228 7.07107e-05 -0.815843
0.316228 0.000141421 -0.815041
0.316228 0.000353553 -0.831606
0.316228 0.000707107 -0.813352
0.316228 0.00141421 -0.728537
0.316228 0.00353553 -0.801706
0.316228 0.00707107 -0.840998
0.316228 0.0141421 -0.397184
0.316228 0.0353553 -0.294861
0.316228 0.0707107 -0.345008
0.316228 0.141421 -0.184061
0.316228 0.353553 -0.180913
0.316228 0.707107 0.164355
0.316228 1.41421 0.458131
0.316228 3.53553 2.60123
0.316228 7.07107 2.60123

3.16228 7.07107e-05 -0.815843
3.16228 0.000141421 -0.815041
3.16228 0.000353553 -0.831606
3.16228 0.000707107 -0.813352
3.16228 0.00141421 -0.728537
3.16228 0.00353553 -0.801706
3.16228 0.00707107 -0.840998
3.16228 0.0141421 -0.397184
3.16228 0.0353553 -0.294861
3.16228 0.0707107 -0.345008
3.16228 0.141421 -0.184061
3.16228 0.353553 -0.180913
3.16228 0.707107 0.164355
3.16228 1.41421 0.458131
3.16228 3.53553 2.60123
3.16228 7.07107 2.60123



==> weight_norm_nesterov_weights_only.tex <==
3.16228e-07 7.07107e-05 0.386962
3.16228e-07 0.000141421 0.406344
3.16228e-07 0.000353553 0.48256
3.16228e-07 0.000707107 0.574903
3.16228e-07 0.00141421 0.700227
3.16228e-07 0.00353553 0.853397
3.16228e-07 0.00707107 0.989069
3.16228e-07 0.0141421 1.12171
3.16228e-07 0.0353553 1.30037
3.16228e-07 0.0707107 1.42569
3.16228e-07 0.141421 1.57434
3.16228e-07 0.353553 1.79581
3.16228e-07 0.707107 1.96035
3.16228e-07 1.41421 2.15178
3.16228e-07 3.53553 2.46829
3.16228e-07 7.07107 2.46829

3.16228e-06 7.07107e-05 0.375998
3.16228e-06 0.000141421 0.403009
3.16228e-06 0.000353553 0.490344
3.16228e-06 0.000707107 0.579938
3.16228e-06 0.00141421 0.709809
3.16228e-06 0.00353553 0.846075
3.16228e-06 0.00707107 0.975645
3.16228e-06 0.0141421 1.0983
3.16228e-06 0.0353553 1.27825
3.16228e-06 0.0707107 1.39198
3.16228e-06 0.141421 1.47607
3.16228e-06 0.353553 1.54606
3.16228e-06 0.707107 1.61295
3.16228e-06 1.41421 1.67067
3.16228e-06 3.53553 1.69414
3.16228e-06 7.07107 1.69414

3.16228e-05 7.07107e-05 0.381475
3.16228e-05 0.000141421 0.406156
3.16228e-05 0.000353553 0.478587
3.16228e-05 0.000707107 0.575147
3.16228e-05 0.00141421 0.684103
3.16228e-05 0.00353553 0.813511
3.16228e-05 0.00707107 0.914102
3.16228e-05 0.0141421 1.01034
3.16228e-05 0.0353553 1.07054
3.16228e-05 0.0707107 1.13891
3.16228e-05 0.141421 1.16914
3.16228e-05 0.353553 1.2093
3.16228e-05 0.707107 1.23847
3.16228e-05 1.41421 1.30621
3.16228e-05 3.53553 1.32411
3.16228e-05 7.07107 1.32411

0.000316228 7.07107e-05 0.36609
0.000316228 0.000141421 0.380757
0.000316228 0.000353553 0.424694
0.000316228 0.000707107 0.498329
0.000316228 0.00141421 0.542839
0.000316228 0.00353553 0.621423
0.000316228 0.00707107 0.653245
0.000316228 0.0141421 0.683281
0.000316228 0.0353553 0.719164
0.000316228 0.0707107 0.745346
0.000316228 0.141421 0.768368
0.000316228 0.353553 0.83077
0.000316228 0.707107 0.834811
0.000316228 1.41421 0.88225
0.000316228 3.53553 1.01288
0.000316228 7.07107 1.01288

0.00316228 7.07107e-05 0.221444
0.00316228 0.000141421 0.151176
0.00316228 0.000353553 0.122682
0.00316228 0.000707107 0.162015
0.00316228 0.00141421 0.204153
0.00316228 0.00353553 0.231489
0.00316228 0.00707107 0.250813
0.00316228 0.0141421 0.283093
0.00316228 0.0353553 0.328953
0.00316228 0.0707107 0.39394
0.00316228 0.141421 0.350043
0.00316228 0.353553 0.489857
0.00316228 0.707107 0.58108
0.00316228 1.41421 0.726085
0.00316228 3.53553 0.707118
0.00316228 7.07107 0.707118

0.0316228 7.07107e-05 -0.357198
0.0316228 0.000141421 -0.303451
0.0316228 0.000353553 -0.241467
0.0316228 0.000707107 -0.220448
0.0316228 0.00141421 -0.201243
0.0316228 0.00353553 -0.181435
0.0316228 0.00707107 -0.135382
0.0316228 0.0141421 -0.0871574
0.0316228 0.0353553 0.0618312
0.0316228 0.0707107 0.0605476
0.0316228 0.141421 0.40147
0.0316228 0.353553 0.205394
0.0316228 0.707107 0.281485
0.0316228 1.41421 0.252967
0.0316228 3.53553 1.42639
0.0316228 7.07107 1.42639

0.316228 7.07107e-05 -0.729212
0.316228 0.000141421 -0.692672
0.316228 0.000353553 -0.634164
0.316228 0.000707107 -0.597846
0.316228 0.00141421 -0.58453
0.316228 0.00353553 -0.599197
0.316228 0.00707107 -0.551301
0.316228 0.0141421 -0.354103
0.316228 0.0353553 0.0610113
0.316228 0.0707107 -0.329718
0.316228 0.141421 -0.31322
0.316228 0.353553 -3.54021
0.316228 0.707107 -1.5
0.316228 1.41421 -1.5
0.316228 3.53553 -1.5
0.316228 7.07107 -1.5

3.16228 7.07107e-05 -0.729212
3.16228 0.000141421 -0.692672
3.16228 0.000353553 -0.634164
3.16228 0.000707107 -0.597846
3.16228 0.00141421 -0.58453
3.16228 0.00353553 -0.599197
3.16228 0.00707107 -0.551301
3.16228 0.0141421 -0.354103
3.16228 0.0353553 0.0610113
3.16228 0.0707107 -0.329718
3.16228 0.141421 -0.31322
3.16228 0.353553 -3.54021
3.16228 0.707107 -1.5
3.16228 1.41421 -1.5
3.16228 3.53553 -1.5
3.16228 7.07107 -1.5


